PLOP: Probabilistic poLynomial Objects trajectory Planning for autonomous driving

To navigate safely in urban environments, an autonomous vehicle (ego vehicle) must understand and anticipate its surroundings, in particular the behavior and intents of other road users (neighbors). Most of the times, multiple decision choices are acceptable for all road users (e.g., turn right or left, or different ways of avoiding an obstacle), leading to a highly uncertain and multi-modal decision space. We focus here on predicting multiple feasible future trajectories for both ego vehicle and neighbors through a probabilistic framework. We rely on a conditional imitation learning algorithm, conditioned by a navigation command for the ego vehicle (e.g., "turn right"). Our model processes ego vehicle front-facing camera images and bird-eye view grid, computed from Lidar point clouds, with detections of past and present objects, in order to generate multiple trajectories for both ego vehicle and its neighbors. Our approach is computationally efficient and relies only on on-board sensors. We evaluate our method offline on the publicly available dataset nuScenes, achieving state-of-the-art performance, investigate the impact of our architecture choices on online simulated experiments and show preliminary insights for real vehicle control

==> CoRL 2020_arXiv/sup_active_testing.tex <==
\section*{Supplementary material: active testing}

\subsection*{Test vehicle}
\label{sec:test-veh}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/d4u_schema.png}
    \caption{Test car setup, with the position of some of the Lidar sensors and the frontal camera (left), and sensor placement and field of view (right)}
    \label{fig:test_setup}
\end{figure}

The test vehicles are two Range Rover Evoque equipped with an industrial sensor suite (see Figure~\ref{fig:test_setup}). For our experiments, we rely on a frontal fisheye camera, situated just above the front license plate, and a 360 degrees array of Lidar sensors. The vehicle past positions are obtained from a high precision GPS and IMU.

During active testing, the predicted ego vehicle trajectory is converted to a steering and acceleration command using a control scheme designed to reach a point 1s in the future. This point is derived analytically from the trajectory polynom. The control algorithm is running on a dSpace microAutobox, and the actuation of pedals and steering wheel is done using a Paravan actuator.


\subsection*{Dataset}

We use the test vehicles (sensor calibration might be slightly different) to record driving data of two different scenarios over a one month period during the summer. First about 100km of driving were recorded in a complex real urban environment which can be challenging in many ways: erased markings, road users bad behavior, hidden signs, crowded streets, pedestrians, etc. The zone of driving was about 3 $km^2$ so each road was taken multiple times. Then 43 km of driving were recorded on a closed urban test track along with another vehicle (see Figure~\ref{fig:teqmo}). This is a less complex scenario in terms of randomness and other road users but denser in terms of signalisation and intersections. To avoid uselessly repetitive recordings over the test track, we used it to practice multiple scenarios such as yield, orange light, roundabout entry/exit, etc.


\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{images/teqmo.png}
    \caption{Aerial view of the test track with typical recording path overlayed}
    \label{fig:teqmo}
\end{wrapfigure}


\subsection*{Ongoing active testing}

Before the pandemic, 2 days of online tests were performed on the test track with encouraging results. Main successes included lane changes, sharp turns, stop and go behind a vehicle and roundabout management. However, issues remained, in particular because of domain shift due to an important weather change between recording and testing.

Online tests in urban scenario have been delayed due to the pandemic situation but will be the focus once the situation improves. We will perform tests with increasing difficulty starting with straight lines and small curves, then going to intersection and traffic lights up to roundabouts \& crowded scenarios.


==> CoRL 2020_arXiv/sup_results.tex <==
We present here a more detailed view of the network architecture, and additional insights on the evaluations of the main article, starting with the open loop scenario on nuScenes and finishing with the closed loop setup.

\section*{Detailed network architecture}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/network_updated.png}
    \caption{Detailed architecture of PLOP neural network}
    \label{fig:network-full}
\end{figure}

Figure~\ref{fig:network-full} shows the precise details of the network architecture of PLOP. In particular, the minimum path to predict the ego trajectory is highlighted: no semantic segmentation, no neighbor trajectories inputs. Note that there is no strict requirement on the image encoder backbone, so the VGG16 could be replaced by another encoder (Resnet, etc).

\newpage

\section*{Detailed results on nuScenes}

In this section, we present a finer analysis of the performance of PLOP on the nuScenes dataset. Other metrics are introduced to better study the behavior of the trajectory prediction. We also present the results of the ablation studies on the network structure. Finally, we present the performance of PLOP on a longer time horizon, in the context of a recent trajectory prediction benchmark of nuScenes.

\subsection*{Additional metrics}

In addition to minADE and minMSD, Final Displacement Error (FDE) (\ref{eq:minfde}) is interesting because it represents how good a method is at reaching a destination regardless of the intermediate path. minFDE is defined as follows:

\begin{align}
\begin{split}
    minFDE &= \frac{1}{N}\sum_{n=1}^{N} \min_{k \in K} ||\mu_{n,k}(T)-\mu_n^*(T)||.
\end{split}
\label{eq:minfde}
\end{align}

It can also be declined into other metrics such as a miss rate where we consider the final position missed if the FDE is greater than a distance threshold.

Planning multiple trajectories implies to select one of them, which cannot be evaluated using the minMSD and minADE metrics. For the neighbors, these metrics might be too lenient: a prediction where one trajectory fits perfectly the ground truth with an extremely low probability and all other trajectories poorly fit the ground truth might be considered as an inaccurate prediction while its minMSD and minADE are close to 0.
% An improvement could be adding a confidence threshold under which trajectories are not considered during metrics computation or considering only top half trajectories ranking them by confidence as in \cite{desire}.
The selection problem is even more complex regarding ego trajectory. If we want to use it for control at some point, we might choose the trajectory with highest confidence given the current navigation command (no orientation issue), or we might try fusing multiple trajectories with high confidence into a safer one. To account for this, we also study the additional metrics confMSD, confADE and confFDE setting $k = \argmax_{k \in K} \pi_k$ in the corresponding equations to evaluate the relevance of the predicted confidence.
We also study \textit{weightFDE} (for weighted-FDE), defined as:

\begin{equation}
    weightFDE = \frac{1}{N}\sum_{n=1}^{N} \sum_{k=1}^{K} \pi_k ||\mu_{n,k}(T)-\mu_n^*(T)||.
\end{equation}

The goal of weightFDE is to check if high weight trajectory components also have a high error. Comparing it to confFDE highlights how alternative trajectories with non maximum weights compare to the most confident trajectory.

Finally, splitting the metrics regarding to the longitudinal axis $x$ or the lateral axis $y$ is also relevant. Depending on the situation an error on the $x$ axis might be negligible or on the contrary very significant compared to the same error on the $y$ axis.

\subsection*{Finer analysis on offline metrics}

\begin{figure}[t]
    \centering
    \begin{subfigure}{.4\textwidth}
      \centering
      % include first image
      \includegraphics[width=1.0\columnwidth]{images/ego_pond_vs_min_vs_best.png}
      \caption{Ego Vehicle}
      \label{fig:ego_conf_min}
    \end{subfigure}%
    \begin{subfigure}{.4\textwidth}
      \centering
      % include second image
      \includegraphics[width=1.0\columnwidth]{images/nbrs_pond_vs_min_vs_best.png}
      \caption{Neighbor Vehicles}
      \label{fig:nbrs_conf_min}
    \end{subfigure}

 \caption{Comparison between the $conf$, $weight$ and $min$ metrics. On both figures, the axis $x$ represents a threshold value in meters and on the $y$ axis value we report the accumulated percentage trajectories verifying $confFDE < x$, $weightFDE < x$ and $minFDE < x$ over the test set. Figure~\ref{fig:ego_conf_min}, resp. \ref{fig:nbrs_conf_min}, presents the results obtained for the ego vehicle only, resp. the neighbors only.}
 \label{fig:best_vs_min}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{subfigure}{.4\textwidth}
      \centering
      % include first image
      \includegraphics[width=1.0\columnwidth]{images/ego_pond_best_vs_min_x.png}
      \caption{FDE over $x$ axis}
      \label{fig:ego_conf_min_x}
    \end{subfigure}%
    \begin{subfigure}{.4\textwidth}
      \centering
      % include second image
      \includegraphics[width=1.0\columnwidth]{images/ego_pond_best_vs_min_y.png}
      \caption{FDE over $y$ axis}
      \label{fig:ego_conf_min_y}
    \end{subfigure}

 \caption{Variations of FDE between the longitudinal and lateral axis. Plots are similar to \ref{fig:ego_conf_min}. The plot \ref{fig:ego_conf_min_x}, resp. \ref{fig:ego_conf_min_y}, compares the $minFDE$, $weightFDE$ and $confFDE$ metrics regarding the longitudinal axis, resp. the lateral axis, for the ego vehicle over the test set.}
 \label{fig:ego_conf_min_xy}
\end{figure}

We study the performance differences between the most confident trajectory, the confidence weighted sum of predictions and the closest to the ground truth trajectory using $conf$, $weight$ and $min$ metrics. The detailed comparison is presented in Figure \ref{fig:best_vs_min}: by definition $min$ yields better results that $conf$ and $weight$. 
% The curves show that using the confidence as a selector for trajectory planning is relevant.
For the neighbors, we note that the gap between the $min$ and $conf/weight$ curves is not closing up even when the FDE reaches 7m. This result exhibits the variety of behaviors in the predicted trajectories since similar behaviors have similar trajectories and vice versa. This result is not observed for the ego vehicle because it is conditioned by a navigation command.
 
Figure~\ref{fig:ego_conf_min_xy} illustrates the difference for the FDE metrics between $x$ and $y$ axis. We can see that FDE is significantly lower for $y$ than $x$. Even if ideally both errors should be as low as possible, we have to consider that the lateral error is the most critical for control and prediction.

\subsection*{Ablation studies on offline metrics}

To study the impact of our design choices, ablation studies are conducted on our network structure, both for inputs and auxiliary outputs. All networks are trained for a fixed number of 60 epochs. The full architecture is used as a benchmark architecture, and the following components are removed: Lidar input, camera input, semantic segmentation auxiliary loss, % setting $\alpha=1$ parameter of loss $L_{\mathtt{NLL}}$,
and finally multimodal trajectories (predicting only one single trajectory for each vehicle with $K=1$).
% , using the same polynomial formulation as the $(\mu_{k,x}(t), \mu_{k, y}(t))$.

The results are presented in Table~\ref{tab:ablation} where each ablation row has to be compared to the \textit{Full} top row.
The ablation of the auxiliary semantic loss worsens the metrics for ego vehicle. It shows that teaching the network to represent such semantic in its features improves the prediction. This ablation also brought more instability during the training process.
Removing the camera does not yield results as poor as we could have expected for the ego vehicle trajectory planning, even if we cut out very useful information about the current scene like road markings, traffic light states, traffic signs, etc. An explanation could be the passivity of the testing method that does not penalize enough reactive behaviors (e.g. braking when the positions history is braking).
It would not be reasonable to cut out this kind of information in a real self driving car.
The two previous ablations also removed diversity in the observed data since they do not use the Audi semantic dataset for training. However, A2D2 also brings in some bias since it contains only right-hand drive data when nuScenes contains both: righ-hand and left-hand drive data.
We observe that removing the Lidar point cloud degrades all metrics, especially for the neighbors. This result was expected because we removed a lot of useful information about the free space of the static scene.
Using $K=1$ approach yields very poor results, also visible in the training loss. It was an anticipated outcome due to the ambiguity of human behavior.

Finally, the detailed impact of the number of components on minFDE can be visualized in Figure~\ref{fig:multitraj}. The results are consistent with those shown in Table~3 of the main article: adding new component has a positive yet decreasing impact on the performance. Interestingly, the difference is much steeper on the y axis than the x axis. This might be because there can be much more lateral variability on trajectories when at an intersection: in this kind of situations, more trajectories are required to model the possible behaviors.

\begin{table}
\centering
\begin{tabular}{c|cc|cc}
\toprule
 & \multicolumn{2}{c}{Ego vehicle} & \multicolumn{2}{c}{Neighbor vehicles} \\
 \midrule
 & minMSD & minADE & minMSD & minADE \\
\midrule
Full & \textbf{1.65} & 0.79 & \textbf{2.82} & \textbf{0.88}\\
No segmentation & 1.68 & \textbf{0.77} & 2.91 & 0.95\\
No camera & 1.72 & \textbf{0.77} & 2.95 & 0.90 \\
No Lidar & 1.80 & 0.81 & 3.02 & 0.93 \\
$K=1$ & 4.13 & 1.26 & 9.91 & 1.83\\
%Deterministic L2 & 4.23 & 1.31 & 9.81 & 1.90\\
\bottomrule
\end{tabular}
\caption{Ablation study metrics for component removal.}
\label{tab:ablation}
\end{table}

\begin{figure}[t]
    \centering
    \begin{subfigure}{.4\textwidth}
      \centering
      % include first image
      \includegraphics[width=1.0\columnwidth]{images/multitraj_ego.png}
      \caption{Ego Vehicle}
      \label{fig:ego_min_multitraj}
    \end{subfigure}%
    \begin{subfigure}{.4\textwidth}
      \centering
      % include second image
      \includegraphics[width=1.0\columnwidth]{images/multitraj_nbrs.png}
      \caption{Neighbor Vehicles}
      \label{fig:nbrs_min_multitraj}
    \end{subfigure}

 \caption{Impact of the number of predicted trajectories $K$. Plots are similar to Figure~\ref{fig:best_vs_min}. The plot \ref{fig:ego_min_multitraj}, resp. \ref{fig:nbrs_min_multitraj}, presents the results obtained over the test set comparing the $minFDE$ performance using multiple values of $K$ for the ego vehicle only, resp. the neighbor vehicles only.}
 \label{fig:multitraj}
\end{figure}



\subsection*{Longer time horizon}

Recently, a benchmark on trajectory prediction has been introduced on the nuScenes dataset \footnote{\url{https://www.nuscenes.org/prediction?externalData=all&mapData=all&modalities=Any}}. This benchmark evaluates neighbors trajectory predictions over a 6s time horizon. Up to 25 future trajectories (\textit{modes}) can be proposed, and the following metrics are used: minimum ADE, FDE, miss rate at 2m (whether the predicted final point is in a 2m range of the ground truth). These metrics can be evaluated for the top $k$ modes, with $k=1, 5, 10$ (although only part of these results is publicly available, see Table~\ref{tab:nuscenes_6s}).

Our method is trained as described in the main paper, extending the prediction horizon to 6s (which means $T=60$), with the same number of maximum trajectories $K=12$. Trajectories are ranked according to their GMM weights $\pi_k$. Objects that are out of the input birdview range are predicted using the constant velocity baseline. We report our results in Table~\ref{tab:nuscenes_6s}. Note that this is far from ideal for our approach: a single polynomial of degree 4 is not enough to represent precisely represent such a long time horizon. Typically, the mean ADE between the ground truth positions and the polynomial fitting is around 0.6m, whereas for 4s it is around 0.2m.

\begin{table}[t]
    \centering
    \begin{tabular}{c|ccccccccc}
    \toprule
         & \multicolumn{3}{c}{minADE (m)} & \multicolumn{3}{c}{minFDE (m)} & \multicolumn{3}{c}{Miss rate (\%)} \\
         Top $k$ & $k = 1$ & $k=5$ & $k = 10$ & $k = 1$ & $k=5$ & $k = 10$ &  $k = 1$ & $k=5$ & $k = 10$ \\
         \midrule
         PLOP & 2.793 & 2.080 & 1.899 & \textbf{6.783} & 4.580 & 3.951 & 52.85 & 51.39 & \textbf{50.91} \\
         cxx & - & \textbf{1.630} & 1.288 & 8.865 & - & - & - & 68.95 & 60.47 \\
         MHA-JAM & - & 1.813 & \textbf{1.241} & 8.569 & - & - & - & 59.15 & \textbf{45.61}\\
         Physics oracle & - & 3.70 & 3.70 & 9.09 & - & - & - & 88.0 & 88.0 \\
         \bottomrule
    \end{tabular}
    \caption{Comparison over the nuScenes prediction benchmark: our approach (PLOP) compared to the top 2 rankings of the nuScenes prediction challenge (cxx and MHA-JAM) and a physical car model baseline.}
    \label{tab:nuscenes_6s}
\end{table}

For comparison, we present the results of the top 2 competitors at the time of submission (according to ADE and FDE): cxx \citep{luo2020probabilistic} and MHA-JAM \citep{messaoud2020multi}. Both methods rely on HD maps input. We also include the baseline \textit{Physics oracle} which is a trajectory prediction model that models the dynamics of the vehicle (more complex than the constant velocity baseline). Interestingly, PLOP is comparable to HD maps based methods. As expected, PLOP has worse results in $minADE$, which represents the general fitting of the trajectory. However, PLOP improves over both other methods in $minFDE$ and is competitive for miss rate, which shows that our approach can get better results on the final position estimation. We hypothesize that this is due to the fact that our prediction approach is single shot: the polynomial representation might be better at capturing the long term dynamic of the trajectory, at the cost of an approximation locally on the individual points. In contrast, sequential methods accumulate errors over time and do not have a global correction mechanism in the loss to compensate.

\newpage

\section*{Additional results on online simulation}

In this section, we give more details on the network input in the real vehicle setup. Then we add a slightly more detailed analysis of the closed loop simulated failure cases.

\subsection*{Details on image input}

Figure~\ref{fig:fisheye} illustrates the image input data with more details. Here we present the raw, original fisheye images and compare them with the used cylindrical projection. The fisheye images correspond to 195 degrees of field of view, hence the strong effects of distortion. Note how the lines are straightened in the corresponding reprojection (150 degree field of view). This reprojection is done mainly to compensate for the distortion effects. To visualize the range of visibility in the image, we show lines corresponding to a ground plane projection spaced by 1m. In practice, the effective detection range is around 20-30m.

\begin{figure}[h]
    \centering
    \subfloat[Original fisheye image]{\includegraphics[width=0.45\textwidth]{images/fisheye_orig.png}}
    \qquad
    \subfloat[Corresponding cylindrical reprojection]{\includegraphics[width=0.45\textwidth]{images/cyl_orig.png}} \\
    \subfloat[Metric graduation on the original fisheye image]{\includegraphics[width=0.45\textwidth]{images/fisheye_withpos.png}}
    \qquad
    \subfloat[Metric graduation on the cylindrical image]{\includegraphics[width=0.45\textwidth]{images/cyl_withpos.png}}
    \caption{Details on image input: original image vs cylindrical reprojection input, and visualization of detection range: $x \in [0.5; 20.5]m$ every 1m (blue dashed lines) and $y \in [-10; 10]m$ every 1m (red dashed lines)}
    \label{fig:fisheye}
\end{figure}

Using a fisheye camera is what makes it possible to generate deviations from the expert trajectories to correctly train the network with IL. This method is following the approached proposed by \citet{lat_fisheye} to generate the input images corresponding to deviations. For the Lidar data, the generation is much simpler as it is equivalent to a reference change in the point cloud. The drawback is that such cameras have a limited range, which advocates for the use of Lidar to compensate.

\subsection*{Closer analysis of closed loop failure cases}

In Figure~\ref{fig:vs_no_seg} we present a detailed comparison between PLOP and PLOP trained without the semantic segmentation auxiliary loss. As seen in the main article, the online metrics are worse without the semantic segmentation. Interestingly, lateral errors seem to occur in difficult cases (hard turns, roundabout) without the semantic segmentation.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[height=4cm]{images/urban_plop.png}
    \caption{PLOP, urban}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[height=4cm]{images/plop_nosem_urban.png}
    \caption{PLOP no seg., urban}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[height=4cm]{images/track_plop.png}
    \caption{PLOP, track}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[height=4cm]{images/plop_nosem_track.png}
    \caption{PLOP no seg., track}
    \end{subfigure}
    \caption{Closed loop error locations for urban and track test data, visualized for PLOP with or without semantic segmentation (no seg.) baseline. 
    %We note that due to the simulator design, high speed errors can occur multiple times in the same situation explaining the difference between the results presented in Table~\ref{tab:baseline_comparison} and the number of red dots.
    }
    \label{fig:vs_no_seg}
\end{figure}

Figure~\ref{fig:detailed_track} shows a more detailed view of the comparison of PLOP versus our baselines on the track setup. As expected, our baselines fail to stop at traffic lights and stop signs (high speed errors), because the input does not contain any information on the traffic light status. Interestingly, we can see that the failure cases for the lateral behavior are not the same between constant velocity and MLP prediction: in the constant curves (the large roundabout and the top-right curve), MLP actually manages to keep the vehicle in the lane, but fails on the speed. This is probably because the MLP is able to produce curved trajectories, but is not able to distinguish the driving speed between a sharp turn and a roundabout. 

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[height=5cm]{images/track_plop.png}
    \caption{PLOP}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[height=5cm]{images/track_cv.png}
    \caption{Constant velocity}
    \end{subfigure}
     \begin{subfigure}{0.3\textwidth}
    \includegraphics[height=5cm]{images/track_mlp.png}
    \caption{MLP}
    \end{subfigure}
    \caption{Detailed comparison of failure cases on track}
    \label{fig:detailed_track}
\end{figure}

Figure~\ref{fig:failure_images} presents some qualitative examples of typical failure cases, where the speed predicted by PLOP is too high. Most braking errors come from difficult traffic lights, harder vehicles (trucks), or difficult use cases (non careful pedestrian). In future work, adding more cameras, typically from the side mirrors, might mitigate some of these use cases.

\begin{figure}[h]
    \centering
    \subfloat[Missed traffic light (on track) due to sun glare.]{\includegraphics[width=0.45\textwidth]{images/high_speed_0.png}}
    \qquad
    \subfloat[Missed braking on a rare event of a truck stopped on roundabout.]{\includegraphics[width=0.45\textwidth]{images/high_speed_1.png}} \\
    \subfloat[Missed braking due to a sudden pedestrian crossing (far right).]{\includegraphics[width=0.45\textwidth]{images/high_speed_2.png}}
    \qquad
    \subfloat[Missed traffic light due to sun glare / partial obstruction by leaves.]{\includegraphics[width=0.45\textwidth]{images/high_speed_3.png}}
    \caption{Qualitative examples of failure cases because of high predicted speed (raw fisheye image)}
    \label{fig:failure_images}
\end{figure}

